On the Efficiency and Robustness of Vibration-based Foundation Models for IoT Sensing: A Case Study

This paper demonstrates the potential of vibration-based Foundation Models (FMs), pre-trained with unlabeled sensing data, to improve the robustness of run-time inference in (a class of) IoT applications. A case study is presented featuring a vehicle classification application using acoustic and seismic sensing. The work is motivated by the success of foundation models in the areas of natural language processing and computer vision, leading to generalizations of the FM concept to other domains as well, where significant amounts of unlabeled data exist that can be used for self-supervised pre-training. One such domain is IoT applications. Foundation models for selected sensing modalities in the IoT domain can be pre-trained in an environment-agnostic fashion using available unlabeled sensor data and then fine-tuned to the deployment at hand using a small amount of labeled data. The paper shows that the pre-training/fine-tuning approach improves the robustness of downstream inference and facilitates adaptation to different environmental conditions. More specifically, we present a case study in a real-world setting to evaluate a simple (vibration-based) FM-like model, called FOCAL, demonstrating its superior robustness and adaptation, compared to conventional supervised deep neural networks (DNNs). We also demonstrate its superior convergence over supervised solutions. Our findings highlight the advantages of vibration-based FMs (and FM-inspired selfsupervised models in general) in terms of inference robustness, runtime efficiency, and model adaptation (via fine-tuning) in resource-limited IoT settings.

==> tables/direct_inference.tex <==
\begin{table}[]
\centering
\caption{Inference Results. Models are trained/fine-tuned on the MOD dataset.}
\label{tab:direct_inference}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}cc|cc|cc|cc@{}}
\toprule
\multicolumn{2}{c|}{\textbf{Dataset}} & \multicolumn{2}{c|}{\textbf{MOD}} & \multicolumn{2}{c|}{\textbf{\firstday}} & \multicolumn{2}{c}{\textbf{Noisy Set}} \\ \midrule
\multicolumn{1}{c|}{Encoder}                    & Framework  & Acc    & F1     & Acc    & F1     & Acc    & F1     \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{DeepSense}} & Supervised & 0.9404 & 0.9399 & 0.4716 & 0.4313 & 0.4611 & 0.4746 \\
\multicolumn{1}{c|}{}                           & FOCAL      & 0.9732 & 0.9729 & 0.4467 & 0.4059 & 0.5613 & 0.5525 \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{SW-T}}      & Supervised & 0.8948 & 0.8931 & 0.4086 & 0.3976 & 0.4543 & 0.4589 \\
\multicolumn{1}{c|}{}                           & FOCAL      & 0.9805 & 0.9800 & 0.4365 & 0.3937 & 0.5311 & 0.5186 \\ \bottomrule
\end{tabular}%
}
\end{table}
